Securing Transformer-based AI Execution via Unified TEEs and Crypto-protected Accelerators

Recent advances in Transformer models, e.g., large language models (LLMs), have brought tremendous breakthroughs in various artificial intelligence (AI) tasks, leading to their wide applications in many security-critical domains. Due to their unprecedented scale and prohibitively high development cost, these models have become highly valuable intellectual property for AI stakeholders and are increasingly deployed via machine learning as a service (MLaaS). However, MLaaS often runs on untrusted cloud infrastructure, exposing data and models to potential breaches. Mainstream protection mechanisms leverage trusted execution environments (TEEs) where confidentiality and integrity for secretive data are shielded using hardware-based encryption and integrity checking. Unfortunately, running model inference entirely within TEEs is subject to non-trivial slowdown, which is further exacerbated in LLMs due to the substantial computation and memory footprint involved. Recent studies reveal that the hybrid TEE-based scheme offloading partial model inference operations to the untrusted accelerators (e.g., GPU) is a promising solution. However, prior offloading schemes fail to ensure dual protection of data and model in Transformer inference, as they cannot securely offload critical operations, i.e., Attention and SoftMax, forcing these computations to remain confined within TEEs. To address these challenges, we propose TwinShield, a framework enabling secure Transformer inference in heterogeneous TEE and accelerator systems with dual protection for both model and data. TwinShield offloads ~87% of computation to GPUs and delivers 4.0x - 6.1x speedups over previous approaches across various Transformer models.

==> sections/5_security.tex <==
% \newpage
% \appendix

% \subsection{Security Analysis of \OutAttenMul{}}
% \label{s:security_attenmul}

% For the transformed $\widetilde{Q}$ and $\widetilde{K^T}$, let $F(\widetilde{Q})$ and $F(\widetilde{K^T})$ represent the set of original matrixs that could have been transformed to $\widetilde{Q}$ and $\widetilde{K^T}$, i.e., the set of possible pre-images for $\widetilde{Q}$ and $\widetilde{K^T}$. We call them \textit{feasible set} for $\widetilde{Q}$ and $\widetilde{K^T}$. The construction of \textit{feasible set} can be found in appendix~\ref{app:feasible_set}.

% \noindent \textbf{Theorem 1.} For a $\widetilde{QK^T}$ computation and a given view of the GPU $\text{View}_{\text{GPU}}=(\widetilde{Q}, \widetilde{K^T}, \widetilde{QK^T}, (QK^T)')$, where \((QK^T)'\) is used to operate subsequent computation in GPU, has been transformed by TEE. We have:
% \begin{equation}
% \label{e:Q}
%     \begin{gathered}
%     \forall (Q_i,Q_j) \in \mathcal{F}(\widetilde{Q})\times \mathcal{F}(\widetilde{Q}) \\
%     \text{Pr}[Q=Q_i|\text{View}_{\text{GPU}}]=\text{Pr}[Q=Q_j|\text{View}_{\text{GPU}}]
%     \end{gathered}
% \end{equation}

% and

% \begin{equation}
% \label{e:K}
%     \begin{gathered}
%     \forall (K^T_i,K^T_j) \in \mathcal{F}(\widetilde{K^T})\times \mathcal{F}(\widetilde{K^T}) \\
%     \text{Pr}[K^T=K^T_i|\text{View}_{\text{GPU}}]=\text{Pr}[K^T=K^T_j|\text{View}_{\text{GPU}}]
%     \end{gathered}
% \end{equation}

% The above theorem states that, on observing transformed input matrices $\widetilde{Q}$ and $\widetilde{K^T}$, output matrix $\widetilde{QK^T}$ and next input matrix $(QK^T)'$, an attacker cannot distinguish between two matrices that belong to its feasible set. Thus, the feasible sets act as cloaking regions for the original matrices.

% \noindent \textit{Proof.} First, we present two helper lemmas as follows.

% \noindent \textbf{Lemma 1.} \textit{Attacker cannot reconstruct $QK^T$ from $\widetilde{QK^T}$ and $(QK^T)'$.} Recall that the attacker (GPU) computes $\widetilde{QK^T}=\widetilde{Q}\cdot\widetilde{K^T}$ and subsequently transmits it to TEE. Within the TEE, $\widetilde{QK^T}$ undergoes a recovery process to $QK^T$ through a specific linear transformation, denoted as $f(\cdot)$. Following this, $QK^T$ is subjected to a masking process via another linear transformation, represented as $g(\cdot)$, resulting in the matrix $(QK^T)'$, which is then relayed back to the GPU for subsequent computations. Given the absence of knowledge regarding the intricacies and parameters of the linear transformations $f(\cdot)$ and $g(\cdot)$ on the part of the attacker, it is postulated that the reconstruction of the intermediate matrix $QK^T$ from the accessible matrices $\widetilde{QK^T}$ and $(QK^T)'$ is not computationally feasible for the adversarial entity. 


% \noindent \textbf{Lemma 2.} \textit{Random masked vectors \(r_i \in R_Q\) or \(r_j \in R_K\) are indistinguishable from transformed vectors $q_i \in Q$ or $k_j \in K$ which are the same shape.} Note that $\widetilde{Q}$ and $\widetilde{K^T}$ are embedded in a field $\mathbb{F}$. Thus clearly, masking the inputs is equivalent to applying a one-time pad~\cite{katz2007introduction}. And the \(\widetilde{Q}\) and \(\widetilde{K^T}\) are permuted before sending to GPU.

% % Clearly, these two lemmas state the attacker cannot either obtain information from the output or input. So they don't have any instruction to know which one in feasible set is more likely to be the pre-images $Q$ or $K^T$, as the Equation~\ref{e:Q} and~\ref{e:K} shows.


% \noindent \textbf{Theorem 2.} Given the intricacies of the transformation process applied to the $n$-dimension matrix $X$, we can quantify the probability of correctly deducing the original matrix from its transformed version by the attacker. This quantification is simplified under certain assumptions, notably regarding the scalar coefficients used in the transformation. The theorem assumes these scalar coefficients are integers constrained within the range $(-L,L)$. This simplification is a significant factor in calculating the overall probability and is chosen for its practicality in mathematical modeling and computation.



% \begin{equation}
% \text{Pr[Correct]} = \frac{\binom{n}{n}}{\binom{2n}{n}} \times \left(\frac{1}{2n-n}\right)^n \times \left(\frac{1}{2L}\right)^n \times \frac{1}{n!}
% \label{e:verify_outmul}
% \end{equation}

% This equation encapsulates the aggregate probability, taking into account various factors including the selection of the correct vectors, identification of corresponding masks, accurate prediction of scalar coefficients, and the reordering of the shuffled matrix.


% \noindent \textit{Proof.}
% The proof of Theorem 2 integrates the factors influencing the overall probability of an attacker correctly guessing the original matrix $X$. The probability is derived from the combination of several factors:
% \begin{enumerate}
%     \item Selection of Original Vectors: The correct identification of the original $n$ vectors from a total of $2n$ vectors is represented by the combinatorial ratio $\frac{\binom{n}{n}}{\binom{2n}{n}}$, indicating the statistical likelihood of choosing the exact subset of original vectors.
%     \item Mask Identification: In the obfuscation process, correctly identifying the appropriate masks from the remaining $n$ vectors has a probability of $\left(\frac{1}{2n-n}\right)^n$, assuming each choice is independent and uniform.
%     \item Scalar Coefficients: The scalar coefficients, which are integers within the range $(-L,L)$, have a uniform probability distribution. Thus, the probability of correctly guessing all coefficients is $\left(\frac{1}{2L}\right)^n$.
%     \item Order Recovery: The likelihood of correctly re-establishing the original sequence in the shuffled matrix is represented by the permutation probability $\frac{1}{n!}$.
% \end{enumerate}

% \subsection{Security Analysis of \OutSoftMax{}}
% \label{s:security_uverify}
% Given the transformed vector \(X' = [x_1-r_1, ..., x_i-r_i]\), it is infeasible for an attacker to recover the original vector \(X = [x_1, x_2, ..., x_i]\). The level of security is guaranteed by the additive secret sharing~\cite{cramer2015ass, demmler2015ass2} which assumes that the attacker lacks knowledge of the random vector \([r_1, r_2, ..., r_i]\), which are essential for the reconstruction of the original vector.

% \subsection{Security Analysis of \UVerify{}}
% \subsubsection{verification of \OutSoftMax{}}
% Given the vector share of the GPU \([x_1-r_1,...,hashX-r_{hash},...,x_n-r_n]\), GPU is expected to return \([e^{x_1-r_1},...,e^{hashX-r_{hash}},...,e^{x_n-r_n}]\). Consider three types of attack:

% (a) the attacker tampers the results to 
% \begin{equation}
%     [e^{x_1-r_1+\Delta_1},...,e^{hashX-r_{hash}},...,e^{x_n-r_n}]
% \end{equation}

% (b) the attacker tampers the results to 
% \begin{equation}
%     [e^{x_1-r_1}+\Delta_1,...,e^{hashX-r_{hash}},...,e^{x_n-r_n}]
% \end{equation}

% (c) the attacker swap the positions of different elements.

% According to the verification process in Equation~\ref{e:hash_r}, the TEE will check if:



% \begin{equation}
%     \left(e^{x_1+\Delta_1}\right)^{a_1}\prod_{i=2}^{n} (e^{x_i})^{a_i} = e^{hashX}
% \label{e:hash_r}
% \end{equation}

% For the attack (a), the attacker needs also change:
% \begin{equation}
%     e^{hashX-r_{hash}} \rightarrow e^{hashX-r_{hash}}e^{\Delta_1a^1}
% \end{equation}

% So it is crucial to discern the index of \(hashX\) as well as the coefficients \(a_i\) that the TEE uses for verification of \(x_i\) in Equations~\ref{e:hash} and~\ref{e:hash_r}.

% \noindent\textbf{Lemma 3.} \textit{Given the vector \([x_1-r_1, ..., hashX - r_{hash},...,x_n-r_n]\), \(hashX - r_{hash}\) is indistinguishable from any transformed \(x_i-r_i\).} Since \(x_i-r_i\) and \(hashX - r_{hash}\) are embedded within a field \(\mathbb{F}\) and the \(hashX - r_{hash}\) is inserted by the TEE in an obfuscated location.


% \noindent \textbf{Theorem 3.} Building upon Lemma 3, we can determine the probability of an attacker successfully tampering with \(k\) bits using attack (a) of an \(n\)-dimensional vector without detection by \(\text{\UVerify{}}\):
% \begin{equation}
%     \text{Pr[Correct]} = \frac{1}{n} \times \left(\frac{1}{2L}\right)^k
% \end{equation}
% The factor \(\frac{1}{n}\) reflects the probability of accurately identifying \(hashX\), echoing the premise of Lemma 3. The following term, \(\left(\frac{1}{2L}\right)^k\), represents the probability of correctly guessing all \(k\) coefficients \(a_i\), where these coefficients are integers sampled from the interval \((-L, L)\).

% For attack (b), the tampered item \(e^{x_1-r_1}+\Delta_1\) will first be multiplied by \(e^{r_1}\) during the verification in TEE, and then the TEE will check if:

% \begin{equation}
%     \left(e^{x_1}+\Delta_1e^{r_1}\right)^{a_1}\prod_{i=2}^{n} (e^{x_i})^{a_i} = e^{hashX}
% \label{e:hash_r}
% \end{equation}

% so the attacker needs also know the \(r_1\), \(a_1\) and \(e^{x_1}\) to successful attack. The success probability is:

% \begin{equation}
%     \text{Pr[Correct]} = \frac{1}{n} \times \left(\frac{1}{2L}\right)^k \times \left(\frac{1}{2L}\right)^k \times \left(\frac{1}{2L}\right)^k
% \end{equation}

% For attacker (c), because the secret vector \(\boldsymbol{a}\) will used in the integrity check as Equation~\ref{e:hash_r}, any mismatch of \(a_i\) and \(x_i\) will leads to the failure verification in Equation~\ref{e:hash_r}.

% \subsubsection{verification of \OutAttenMul{} In the \UVerify{} process, the TEE first generates \(hashQ\) as Equation~\ref{e:verify_mul}, and then outsources the concatenated matrix by \OutAttenMul{}. The security are guaranteed by the lower probability of identify the \(hashQ\) from the \(\widetilde{Q}\) quantized in Equation~\ref{e:verify_outmul}. Upon the assumption that the attacker cannot identify the \(hashQ\), the integrity are guaranteed using the variants of an algorithm by Freivalds~\cite{freivalds1977probabilistic}. 

% \noindent\textbf{Theorem 4.} (Freivalds) \textit{Let \(Q\), \(K^T\) and \(Z\) be \(n\times n\) matrices on over a field \(\mathbb{F}\) and let \(s\) be a uniformly random vector in \(\mathbb{S}\subseteq\mathbb{F}\). Then \(\text{Pr}[sZ=(sQ)K^T|Z\neq QK^T]=\text{Pr}[s(Z-QK^T)=0|(Z-QK^T)\neq 0]\leq \frac{1}{|\mathbb{S}|}\)}.

% \label{s:security_uverify}
